Transformer-Squared: Self-adaptive LLMs

Self-adaptive large language models (LLMs) aim to solve the challenges posed by traditional fine-tuning methods, which are often computationally intensive and static in their ability to handle diverse tasks. We introduce Transformer-Squared, a novel self-adaptation framework that adapts LLMs for unseen tasks in real-time by selectively adjusting only the singular components of their weight matrices. During inference, Transformer-Squared employs a two-pass mechanism: first, a dispatch system identifies the task properties, and then task-specific 'expert' vectors, trained using reinforcement learning, are dynamically mixed to obtain targeted behavior for the incoming prompt. Our method consistently outperforms ubiquitous approaches such as LoRA, with fewer parameters and greater efficiency. Furthermore, Transformer-Squared demonstrates versatility across different LLM architectures and modalities, including vision-language tasks. Transformer-Squared represents a significant leap forward, offering a scalable, efficient solution for enhancing the adaptability and task-specific performance of LLMs, paving the way for truly dynamic, self-organizing AI systems.

==> sections/sec6_ack.tex <==
\ificlrfinal

\section{Author contributions}

Yujin Tang initiated the project.
Qi Sun proposed the prompted-based method, developed the evaluation framework, conducted the experiments, and provided contributions to writing.
Edoardo Cetin designed the few-shot CEM adaptation strategy, performed the experiment, and made major contributions to manuscript writing.
Yujin Tang proposed the core algorithm, conducted initial experiments, made major contributions to the manuscript, and managed the project.

\fi

==> sections_ws/conclusions.tex <==
\section{Conclusion}
\label{sec:conclusion}
\vspace{-2mm}

We introduced \implname, a novel blueprint toward realizing self-adaptive LLMs. 
We first proposed \svdacro, offering superior performance, reduced costs, high compositionality, and overfitting regularization. 
Building on \svdacro experts, we developed three effective self-adaptation strategies, each providing unique benefits and scalable performance improvements. 
Future work could explore cross-model compatibility and expert skill recycling across model generations, drawing from recent model merging techniques~\citep{yu2024language,goddard2024arcee,akiba2024evolutionary} to overcome individual LLM limitations.

==> sections_ws/experiments.tex <==
\section{Experiments}
\label{sec:experiments}
\vspace{-2mm}

\subsection{Experimental setups}
\vspace{-1mm}

To validate the generality of \implname we consider three pre-trained LLMs ranging across different model families and architecture sizes: \llama, \mistral, and \llamaXL. 
For each model, we obtain three sets of $z$ vectors to maximize performance for GSM8K~\citep{cobbe2021training},  MBPP-pro~\citep{austin2021program}, and ARC-Easy~\citep{clark2018think}, respectively.
Additionally, we train a set of $z$ vectors for \llama, when applied as the language backbone for TextVQA~\citep{singh2019towards}.
Finally, we evaluate the \implname on four unseen tasks: MATH~\citep{hendrycks2021measuring}, Humaneval~\citep{chen2021evaluating}, ARC-Challenge~\citep{clark2018think}, and OKVQA~\citep{marino2019ok}. 
In our adaptation experiments, we only consider experts obtained in the pure-language settings.
Please refer to Appendix~\ref{app:sec:implementation} for additional details and hyper-parameters summary.

\vspace{-2mm}
\subsection{Experimental results}

\input{tables/svf_train_tasks}


\textbf{\svdacro performance}
resources, with less than 10\% of the training parameters of our LoRA implementation.
We provide results training on each considered task with the \llama, \mistral, and \llamaXL base models in Table~\ref{tab:res:svf_train_tasks}.
Remarkably, we find that \svdacro provides considerable performance gains across nearly all tasks and base models. Instead, LoRA experts yield smaller gains and even sporadic performance degradation.
To ensure a fair comparison, we provide extensive ablations to both our model and the LoRA baseline considering different architecture and optimization objectives in Appendix~ \ref{app:sec:ablation_studies}).


\textbf{Adaptation performance}
With the \svdacro trained $z$ vectors, we assess the self-adaptation capability of \implname on unseen tasks.
As shown in Table~\ref{tab:res:svf_ada_tasks}, all of our \implname adaptation strategies demonstrate improvements across all tasks for nearly all the models.
In contrast, even the best training LoRAs only provide marginal improvements on the ARC-Challenge task and still significantly deteriorate performance on both MATH and Humaneval. 
Comparing the three proposed adaptation strategies, we highlight a clear monotonic trend -- with more involved strategies and additional information about the test-time condition, self-adaptation appears to be increasingly effective.
This trend shows that providing additional or different kinds of information seems to be highly beneficial to our framework, suggesting that \implname could provide foundation models with new means to continually improve performance when deployed in lifelong settings.

\input{tables_ws/svf_ada_tasks}

\vspace{-2mm}
\subsection{Cross-model analysis}
\vspace{-2mm}
\label{sec:analysis}
We explore the potential for our self-adaptation framework to be applied \textit{across different LLMs}. We evaluate whether the \svdacro expert vectors trained on \llama can benefit \mistral, and whether we can perform adaptation across the expert vectors of these two models. We present our main findings in Table~\ref{tab:analysis:cross_model_main} and refer to Appendix~\ref{app:sec:additional_exp} for additional detailed results. 
Surprisingly, positive transfer does occur across the two models, with visible benefits in 2 out of 3 tasks.
We note these improvements are due to the inherent ordering of the \svdacro parameterization, as \textit{randomly shuffling} each \svdacro vector before applying it to the Mistral model consistently degrades performance. 
This operation leads to notable performance degradation across tasks. 
Finally, by performing few-shot adaptation using the \svdacro vectors collected from both models, the performance of \mistral further improves across the board.
We observe that these gains even surpass the best score from adapting \mistral with \textit{all} the \svdacro vectors in the ARC-Challenge task reported in Table~\ref{tab:res:svf_ada_tasks}.  
While these results appear promising, we note that the surprising compatibility discovered through our naive transfer approach is potentially tied to the similarity between the architectures of the two considered LLMs.
To this end, whether similar transfer can be replicated with models of different scales remains an open research question that could open the doors to disentangling and recycling task-specific skills for models, with important implications for the democratization and sustainability of the field.

\vspace{-4mm}
\input{tables_ws/analysis_cross_model_main}

==> sections_ws/introduction.tex <==
\section{Introduction}
\label{sec:introduction}

\begin{wrapfigure}{r}{0.5\textwidth}
\vspace{-6mm}
\begin{center}
    \includegraphics[width=0.5\textwidth]{images/cover.pdf}
  \end{center}
  \vspace{-4mm}
  \caption{\textbf{Overview of \implname.} In training, we tune the singular values of the weight matrices to generate a set of ``expert'' vectors specializing in different tasks. In inference, a two-pass process is adopted where the first applies the expert and the second generates the answer.}
  \label{fig:cover}
  \vspace{-4mm}
\end{wrapfigure}

Self-adaptive large language models (LLMs) would represent a significant advancement in artificial intelligence, enabling real-time adaptation to various tasks and contexts.
While compositionality and scalability are crucial for effective adaptation, current LLM training methodologies fall short of achieving both these properties simultaneously.
Our research aims to present a solution to address these gaps.

In principle, the first step toward achieving self-adaptive LLMs can be realized through the development of specialized expert modules, each fine-tuned~\citep{kaplan2020scaling} via techniques such as low-rank adaptation (LoRA)~\citep{hu2021lora}. 
However, several challenges need to be addressed to make this approach both scalable and compositional: (1) multiple expert modules significantly increase the number of parameters; (2) expert modules are often prone to overfitting; and (3) flexible composition of these experts is still an open problem.

To overcome these limitations, we first propose \svdacro, a novel parameter-efficient fine-tuning (PEFT) method to obtain effective building blocks for self-adaptation.
\svdacro works by extracting and selectively tuning only the singular values within the model's weight matrices.
By focusing on this essential and principled parameterization, our approach mitigates the risk of overfitting, drastically reduces computational demands, and allows for inherent compositionality.

We then introduce our full \implname framework, which entails a two-pass inference mechanism to produce dynamically adapted weights targeted for the test-time conditions (Figure~\ref{fig:cover}).
We design three different adaptation strategies that can be used within \implname, which we show provide monotonic performance benefits with increasing access to the test-time conditions.
We evaluate \svdacro and the full \implname framework through extensive experiments across a diverse range of LLMs and tasks.
\svdacro outperforms traditional efficient fine-tuning methods like LoRA on domain-specific datasets with far fewer parameters. 
\implname further improves performance, even for out-of-distribution tasks like visual QA. 
Our analysis even shows that \implname allows the reuse of \svdacro experts across different LLMs. In summary, our key technical contributions are: 
\vspace{-2mm}
\begin{itemize}
\item The development of \implname as a pivotal self-adaptation framework for LLMs, providing a blueprint to adapt the behavior of LLMs from a growing set of pre-trained skills.
\item The introduction of \svdacro, a novel PEFT method trainable with RL on small datasets, producing compact expert vectors with inherent compositionality.
\item The implementation of three adaptation strategies, effectively dispatching \svdacro-trained experts with properties designed to cope with different deployment scenarios.
\end{itemize}

\vspace{-2mm}

==> sections_ws/methods.tex <==
\section{Methods}
\label{sec:methods}

\vspace{-2mm}
\subsection{Preliminaries}

\textbf{Singular value decomposition (SVD)} offers a fundamental view of matrix multiplications.
In neural networks, each weight matrix $W \in \mathbb{R}^{n \times m}$ can be decomposed into three components $W = U \Sigma V^\intercal$, yielding semi-orthogonal matrices $U \in \mathbb{R}^{m \times r}$ and $V \in \mathbb{R}^{n \times r}$ together with an ordered vector of $r$ singular values arranged in the diagonal matrix $\Sigma \in \mathbb{R}^{r \times r}$.

\textbf{Cross-entropy method (CEM)} is a Monte Carlo method for importance sampling and optimization~\citep{rubinstein2004cross}.
The method is based on minimizing the KL divergence between two probability distributions $D_\mathrm{KL}(P\|Q)$, where $P$ is the target distribution and $Q$ is a maintained distribution. 
CEM generates a set of samples from $Q$, evaluates them, and updates the distribution $Q$ with the characteristics of the elite samples. In the standard setup, $Q$ is set to a diagonal multivariate Gaussian, reducing the problem to simply estimating the empirical mean and standard deviation of the latest elites. We illustrate a complete CEM step in the Python pseudocode in Appendix~\ref{app:sec:fewshot}.

\vspace{-2mm}
\subsection{\textsc{\implname}}
\label{sec:transformer^2}

The construction of \implname comprises two main steps, for which we provide an illustrative overview in Figure~\ref{fig:method_overview}.
First, we introduce \svdname (\svdacro), a method to learn \textit{compositional} expert vectors with RL.
Then, we describe three different adaptation strategies within \implname, inspired by orthogonal principles.
We motivate how the properties of \svdacro are highly complementary to our adaptation strategies, making \implname an effective and scalable framework for the design of new self-adaptive LLMs.

\begin{figure}[!h]
    \centering
    \includegraphics[width=\textwidth]{images/method_overview.pdf}
    \caption{\textbf{Method overview.}
    Left) At training time, we employ \svdacro and RL to learn the ``expert'' vectors $z$'s that scale the singular values of the weight matrices.
    Right) At inference time, we propose three distinct methods to adaptively select/combine the learned expert vectors.
    }
    \label{fig:method_overview}
\end{figure}

\textbf{Singular value fine-tuning}\label{sec:svf} is a key building block in \implname. For any weight matrix $W$, \svdacro learns a simple vector $z\in \R^r$ that provides targeted modifications to each singular component of  $W$ independently, yielding a new weight matrix $W^\prime=U \Sigma^\prime V^\intercal$, where $\Sigma^\prime=\Sigma \otimes\text{diag}(z)$.
This approach offers three main benefits: (1) Negligible parameters: efficient fine-tuning with far fewer optimized parameters than existing methods. 
(2) High compositionality: decomposition into independent singular components enables interpretable $z$ vectors, unlike LoRA-based methods. 
(3) Principled regularization: modifying only pre-existing singular component magnitudes prevents overfitting, allowing fine-tuning on small datasets without risking model collapse. 
These properties make \svdacro a foundation block for adapting large language models efficiently and effectively.

\textbf{End-to-end optimization with RL.} We train a set of \svdacro vectors $\theta_z = \{z_1, \cdots, z_{N \times M}\}$ to fine-tune an arbitrary language model $\pi_{\theta_W}$ parameterized by $\theta_{W}$ with RL, optimizing directly for task performance.
Here, $\theta_{W}=\{ W_1, \cdots, W_{N \times M} \}$ is the set of weight matrices, where $N$ is the number of layers and $M$ is the number of weight matrices to fine-tune per layer.
We use the seminal REINFORCE algorithm~\citep{williams1992simple} and label each generated answer $y_i$ (for the prompt $x_i\in D$) with a unitary reward based on its correctness $r\in \{-1, 1\}$.
Inspired by related applications of RL for optimizing LLMs~\citep{ouyang2022training}, we regularize the REINFORCE objective by adding a KL penalty for deviating from the original model's behavior, weighted by a small coefficient $\lambda \in \mathbb{R^+}$. Thus, our final objective function can be written as:

\begin{equation}
    J(\theta_z) = \E \left[\log\left(\pi_{\theta_{W^\prime}}(\hat{y}_i \mid x_i)\right)r(\hat{y}_i, y_i)\right] - \lambda D_\mathrm{KL}(\pi_{\theta_{W^\prime}} \| \pi_{\theta_{W}}),
\label{eqn:sec3:reinforce}
\end{equation}

where we use $\pi_{\theta_{W^\prime}}$ to denote the resulting language model after substituting the original weight matrices $W$ with $W^\prime$.
While RL is generally considered less stable than next-token prediction objectives, we find the regularization properties of SVF avoid many of the failure modes of prior less-constrained parameterizations (see Section~\ref{app:sec:ablation_studies}).
Thus, combining these complementary components effectively enables us to directly maximize task performance end-to-end.

\textbf{Self-adaptation} is a critical mechanism in nature that has established itself as a core guiding principle in modern system design \citep{7302492}. Our initial efforts toward self-adaptive foundation models focus on the inference stage of LLMs, where we devise a simple two-pass adaptation strategy that combines $K$ sets of base ``expert'' vectors $z^{1:K}$ trained with \svdacro to provide different kinds of capabilities (e.g., coding, math, etc).
In the first inference pass, given an individual input prompt, \implname executes the model and observes its test-time behavior to derive a new $z'$ vector tailored to its test-time conditions. 
This adapted $z'$ is then used in the second inference pass to provide an actual response with the newly adapted weights. 
In this first work, we propose three simple approaches to produce the vector $z'$ during the first inference pass. Below, we provide an outline of each method and refer to Appendix~\ref{app:sec:implementation} for additional implementation details.

\textit{A) Prompt engineering:}
Our most basic approach involves constructing an ``adaptation'' prompt which we use to \textit{ask} the LLM to categorize the input prompt.
Based on its response, we then extract one category out of the set of domain topics used to pre-train each \svdacro expert and, thus, we select the corresponding $z'$ directly from $z^{1:K}$.
We also explicitly provide the option for a generic ``others'' category, allowing the model to use its base weights in case no expert provides appropriate capabilities. We show the format used to construct the adaptation prompt in Appendix~\ref{app:sec:svf}

\textit{B) Classification expert:} 
A direct extension of the prompt engineering approach comes from using a specialized system to handle task identification.
Following the principles of self-adaptation, we apply \svdacro to fine-tune the base LLM itself to handle this task.
In particular, we collect a dataset $D = \{(x_{1,1}, 1), \cdots, (x_{i,k}, k), \cdots \}$ from the $K$ \svdacro training tasks, where $x_{i,k}$ is the $i$-th example from the $k$-th expert task.
Each tuple $(x_{i,k}, k)$ then forms an example to pre-train an additional job classification expert $z^c$ learned in the same fashion as the others.
During the first inference pass, we simply load $z^c$, intending to improve the inherent task classification capabilities of the base model.

\textit{C) Few-shot adaptation:} Our third approach leverages additional task information by assuming extended access to its test-time conditions beyond individual prompts. 
Our method is inspired by few-shot prompting techniques, which have been shown to provide performance improvements, allow LLMs to ``in-context'' learn tasks that were entirely unseen prior to inference~\citep{brown2020language}.
For each optimized $W$, our approach entails producing a new $z^\prime=\sum^{K}_{k=1} \alpha_k z_k$ by linearly interpolating between the $K$ learned \svdacro vectors, each weighted by the coefficients $\alpha_k$.
We employ CEM to search over the $\alpha_k$ based on the performance on a set of ``few-shot prompts'', which are specifically held out from the rest of the test prompts and used to evaluate CEM's population samples. 
In the case of multiple population samples obtaining the same score on these held-out prompts, we break ties by favoring the one with the highest average log-likelihood across its own generated correct answers.
We refer to Section~\ref{app:sec:fewshot}, for additional details and discussions of this final approach. 

\vspace{-2mm}

==> sections_ws/relatedworks.tex <==
\vspace{-1mm}
\section{Related works}
\label{sec:relatedworks}
\vspace{-1mm}
Self-adaptive LLMs operate at macro (multiple collaborating LLMs) and micro (internal adaptations) levels. 
Microview adaptations often use Mixture of Experts (MoE) for dynamic routing~\citep{fedus2022switch}. 
Low-rank adaptation methods like LoRA~\citep{hu2021lora} enable efficient fine-tuning. 
Recent approaches leverage SVD for LLM fine-tuning, either using minor components~\citep{wang2024milora} or top singular vectors~\citep{balazy2024lora}. 
The most related work~\citep{lingam2024svft} explores SVD-based sparsification but doesn't focus on self-adaptive LLMs or use reinforcement learning for efficiency.
We refer to Appendix~\ref{app:sec:extendedrelatedworks} for references to the wider literature.

\vspace{-2mm}

==> sections_ws_app/Aimplementation.tex <==
\section{Implementation details and hyper-parameters}
\label{app:sec:implementation}

\subsection{\svdacro training}
\label{app:sec:svf}
We obtain the expert vectors $z$ as the base components in \implname by training the \svdacro fine-tunes with a consistent recipe across the considered training tasks and language models. 
We divide each dataset to produce equal-sized training and validation splits. We then apply our RL-based approach, optimizing $\theta_z$ with AdamW using a learning rate of $2 \times 10^{-3}$ with cosine decay, a batch size of 256, and gradient clipping. 


\begin{wrapfigure}{r}{0.55\textwidth}
\vspace{-8mm}
\begin{center}
    \includegraphics[width=0.55\textwidth]{images/visualization/system_prompt.pdf}
  \end{center}
  \vspace{-4mm} 
  \caption{\textbf{Prompt based adaptation.} Self-adaptation prompt used by \implname to classify the task prompt into pre-defined categories.}
  \label{app:fig:sys_prompt}
  \vspace{-8mm}
\end{wrapfigure}

We employ early stopping and select the best $\lambda$ (the coefficient of the KL divergence term) based on validation performance. For the \llamaXL and Vision tasks experiments, we apply the \svdacro on half of the layers to reduce memory usage while maintaining considerable performance improvement.
During the training of \llama on the vision language tasks, we apply a small negative reward (-0.1) for training stability.


Our system prompt used for training classification expert is in Figure~\ref{app:fig:sys_prompt}

\subsection{LoRA training}
\begin{wrapfigure}{h}{0.55\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/visualization/ift_math_example.pdf}
   \vspace{-6mm}
  \caption{\textbf{Sample problem and answer.} Math data sample used for LoRA instruction fine-tuning, text in blue is the unmasked solution.}
  \label{app:fig:sft_math_example}
\end{wrapfigure}

We follow community best practices for LoRA fine-tuning, applying it to query and value projection layers with learning rates around $5 \times 10^{-5}$. 
We set 200 total iterations with a 256 global batch size for sufficient training. For feasible LoRA instruction training, we collect solutions for all training tasks (GSM8K, MBPP, Arc-Easy, TextVQA) from official sources and append them to question prompts. 
Table~\ref{app:fig:sft_math_example} shows a sample math problem used for LoRA fine-tuning.
Despite extensive hyperparameter tuning, we often observe test performance decay as discussed, which can be attributed to the small number of training samples and potential model requirements for instruction fine-tuning data (specifically, the highly detailed thinking process).

\subsection{Hyper parameters}
We present a summary of the hyperparameters used in our experiments in Table~\ref{app:tab:hyperparameters}. To optimize performance, we conducted sweeps across several hyperparameters and selected the most effective combination based on validation results.
For \svdacro, our primary focus was on adjusting the KL coefficient to enhance training stability. In the case of LoRA, we concentrated on sweeping the learning rate and maximum gradient clip norm to identify optimal settings.

\input{tables_ws/hyper_p_app}

\subsection{Few-shot adaptation}
\label{app:sec:fewshot}

As described in the main text, our few-shot adaptation approach entails producing an entirely new $z^\prime=\sum^{K}_{k=1} \alpha_k z_k$ for each $W$ by linearly interpolating between the $K$ learned \svdacro vectors, each weighted by the coefficients $\alpha \in \mathbb{R}^K$.
We employ CEM to search for $\alpha_k$'s based on the performance on the few-shot prompts, which are specifically held out from the rest of the test prompts and used to obtain the elite set at each iteration. 
In the case of multiple sample solutions obtaining the same score on these held-out samples, we break ties by choosing the sample solution with the highest average log-likelihood across the tokens of its generated correct answers.

In all of our main experiments we reserve only 10 samples of data for self-adaptation and perform up to 100 CEM iterations. For each setting, we consider both per-layer and per-vector adaptation, where the latter strategy has the advantage of greatly simplifying search (as we only have 3 $\alpha$ coefficients). Moreover, we experiment with both normalizing across the $\alpha$ of different tasks (such that their sum would be fixed to 1) or keeping them unconstrained. Due to the lack of a validation set, we simply report the performance attained by our best sample from these test configurations at the end of optimization, on the remaining unseen samples for each task.

We provide our python pseudo code of one CEM step as follows:
\begin{minted}[framesep=2mm, baselinestretch=1.2, bgcolor=verylightgray, fontsize=\footnotesize]{python}
def cem_step(mu, sigma, num_elites, num_samples):
    samples = np.random.normal(loc=mean, scale=sigma, size=num_samples)
    scores = evaluate(samples)
    elites = samples[np.argsort(scores)[-num_elites:]]
    new_mu = np.mean(elites, axis=0)
    new_sigma = np.std(elites, axis=0)
    return (new_mu, new_sigma)
\end{minted}
\vspace{-10mm}

==> sections_ws_app/BaddExperiments.tex <==
\section{Additional results}
\label{app:sec:additional_exp}


\subsection{Ablation studies}
\label{app:sec:ablation_studies}

\textit{Module sensitivity:} We first compare the performance of \svdacro when it is applied to different modules (see trials 1-3).
Under consistent conditions, both individual MLP and attention updates improve performance, with MLP updates resulting in more pronounced gains.
Simultaneous updates to both module types yield even more significant enhancements.

\textit{Objective function:} We are interested in the performance impact from different objective functions, and we compare the RL objective with next-token prediction loss (see trials 2 and 4).
For the latter, we use instruction fine-tuning with official GSM8K solutions as target tokens.
Results show clear performance gains with RL, demonstrating its effectiveness in task-specific fine-tuning.
Conversely, next-token prediction even hinders performance.
This highlights RL's ability to handle cases lacking detailed solutions, suggesting its superiority in this context.

\textit{\svdacro vs LoRA:} Finally, we also evaluate LoRA using the RL objective (see trials 2 and 5).
A significant performance disparity is observed, primarily attributed to the severe instability of the LoRA training process.
Despite exploring a wide range of learning rates, LoRA's performance consistently lagged behind.
For further illustrations, see Figure~\ref{app:fig:lora_learning_curves} in the appendix.

\input{tables_ws/table_ablation}

\subsection{Impact from number of few-shots}
\label{app:sec:ablation_few_shots}

We investigate the relationship between the number of samples available for few-shot adaptation and downstream performance.
Our analysis focused on the test task where \llama demonstrates the highest baseline performance, to prevent the potential for a null signal in our CEM-based search.

\input{tables_ws/ablation_few_shots}

As Table~\ref{tab:ablation:few_shot_adaptation} shows, substantial benefits of our few-shot strategy are evident with as few as 3 to 5 test samples.
Moreover, performance appears to plateau beyond 10 samples, underscoring how our essential and inherently regularized \svdacro parameterization effectively complements self-adaptation.
This efficiency enables optimal use of data to enhance understanding of the test task.

\subsection{Cross-model svf transfer on the training tasks}
We provide complementary results to Table~\ref{tab:analysis:cross_model_main} in the main text, where we analyze the \svdacro cross-model transfer performance from training on GSM8K, MBPP-pro, and ARC-Easy to our considered test tasks. In Table~\ref{tab:analysis:cross_model_app}, we show the results in the same transfer setting this time evaluating \mistral on the same training tasks where the \llama \svdacro vectors were obtained from. Overall, we recognize a similar trend, albeit with less consistent improvement from the original model (only in 1 out of 3 tasks), but still much higher performance than the randomly shuffled baseline. These results further confirm that the canonical ordering of the \svdacro parameterization is key for cross-model transfer, highlighting once more its inherent suitability to empower self-adaptation.

\input{tables_ws/analysis_cross_model_app}

\subsection{Training curve of LoRA and policy gradient}

Figure~\ref{app:fig:lora_learning_curves} gives the learning curves for LoRA training on the GSM8K task.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.6\textwidth]{images/lora_training_curve.pdf}
    \caption{\textbf{Training LoRA with policy gradient.} The dashed line shows the performance of \llama on the test split. LoRA collapses at the beginning of the training stage and fails to recover, leading to negative effects on test performance. We swept a wide range of learning rates $(2 \times 10^{-4}, 5 \times 10^{-4}, \dots, 2\times 10{-2}, 5\times 10^{-2})$, and all learning curves were similar to the one presented.}
    \label{app:fig:lora_learning_curves}
\end{figure}


==> sections_ws_app/Cinterpretation.tex <==
\section{PCA on llama3 and mistral}
\label{app:sec:pca}

To investigate if the singular components that have the highest singular values are able to capture most of the information of a weight matrix, we conducted Principle Component Analysis (PCA) on the weight matrices in \llama and \mistral (see Figures~\ref{fig:pca_analysis_llama3_8b} and~\ref{fig:pca_analysis_mistral_7b}).
In each figure, we plot the variance that is captured by the top $r$ components across all the layers in each type of modules for a weight matrix $W \in \mathbb{R}^{m \times n}$:
$$\text{ratio} = \frac{\sum_{i=1}^r \sigma_i}{\sum_{j=1}^{\min(m, n)} \sigma_j}$$
Here, $\sigma$'s are the ordered (from largest to smallest) singular values on the weight matrix $W$.
It is easy to see from the figures that when $r=256$, less than 50\% of the variance is captured by these top components on average.
For the MLP layers, this fraction is even lower than 20\%.
On the other hand, the ranks adopted by LoRA-XS or similar methods are much less than 256, resulting in even more information loss and restrictions in their modeling power that relies mostly on these $r$ components.


\begin{figure}[!h]
    \centering
    \includegraphics[width=\textwidth]{images/pca_analysis_llama3-8b.pdf}
    \vspace{-6mm}
    \caption{\textbf{PCA of \llama.} We show the ratio of the variance captured by the top $r$ singular components on the y-axis, and the layer indices on the x-axis. Except for the Query, Key and Value projection matrices, small $r$ values only capture a tiny fraction of variance in singular values in the parameter matrices.}
    \vspace{-4mm}
    \label{fig:pca_analysis_llama3_8b}
\end{figure}


\begin{figure}[!h]
    \centering
    \includegraphics[width=\textwidth]{images/pca_analysis_mistral-7b.pdf}
    \vspace{-6mm}
    \caption{\textbf{PCA of \mistral.} We show the ratio of the variance captured by the top $r$ singular components on the y-axis, and the layer indices on the x-axis. Except for the Query, Key and Value projection matrices, small $r$ values only capture a tiny fraction of variance in singular values in the parameter matrices.}
    \vspace{-4mm}
    \label{fig:pca_analysis_mistral_7b}
\end{figure}

==> sections_ws_app/DextendedRelWorks.tex <==

\newpage
\section{Extended Related works}
\label{app:sec:extendedrelatedworks}


\textbf{Self-adaptive LLMs} We define self-adaptive LLMs as a group of LLMs or a standalone LLM that can evaluate and modify its behavior in response to changes in its operating environment or internal state, without external intervention.
This adaptation can be explored from two perspectives: a macroview, where multiple LLMs collaborate and/or compete, and a microview, where internal adaptations allow a single LLM to specialize in different tasks.

\textit{Macroview:} From this perspective, the system directs queries to LLMs with domain specific expertise, prioritizing outputs from expert models, thereby achieving higher accuracy and task-specific optimization.
Such task-specific ensembles can be realized through various mechanisms: multiple LLMs playing distinct roles and coordinate toward a shared goal~\citep{zhuge2023mindstorms}, engaging in mutual listening and debate~\citep{du2023improving}, or using meticulously crafted prompt constructions~\citep{zhang2024proagent} to integrate knowledge library and skill planning.
Naturally, the improvement in the specialization and adaptive capabilities of individual LLMs in the ensemble enhances the collective performance.
Thus, in this paper, we focus on the microview of self-adaptive LLMs.

\textit{Microview:} MoE in LLMs plays a critical role in this perspective~\citep{ICML2024_MoE}.
In MoE systems, inputs are dynamically routed to a subset of specialized modules or layers (e.g., MLPs) containing domain-specific knowledge~\citep{rajbhandari2022deepspeed,fedus2022switch}.
To reduce inference time, researchers introduce sparsely activated MoE where only a subset of the experts are selected per token~\cite{jiang2024mixtral,qwen_team_2024}.
While it is possible to view \implname loosely as a type of MoE, there are two major differences.
In the aforementioned systems, self-adaptation is achieved through token-level routing, whereas \implname employs a sample-level module selection strategy.
The second difference lies in the construction of expert modules.
In traditional MoE systems, expert modules are either trained from scratch~\citep{fedus2022switch,jiang2024mixtral} or dense models (e.g., upcycling)~\citep{qwen_team_2024,zhu2024llama}, without an auxiliary loss to ensure module specialization.
In contrast, \implname specifically trains expert vectors with RL to acquire domain specific-knowledge, making them true experts.


\textbf{Low-rank adaptation}
PEFT methods such as LoRA~\citep{hu2021lora} works by freezing the original model's parameters and introducing small trainable low-rank matrices for task-specific updates.
It significantly lowers the computational and memory costs while providing performance comparable to full fine-tuning.
Inspired by LoRA's design, various modifications have been proposed~\citep{zhang2023adalora,kopiczko2023vera,liu2024dora,balazy2024lora,huggingface2023svdtraining}.
\implname does not rely on low-rank matrices, and instead scales the singular vectors of the original parameter matrix that span the full rank space.


\textbf{SVD for LLM Fine-tuning}
SVD is increasingly being used as an inductive bias for PEFT in LLMs.
For example, \citet{wang2024milora} decompose a weight matrix and use the minor singular components, associated with noisy or long-tail information, to initialize low-rank matrices for LoRA fine-tuning.
In a similar vein, SVD is employed to approximate an original weight matrix with the top $r$ singular vectors, corresponding to the highest singular values.
A small trainable matrix is then introduced on top of the truncated singular value matrix to adjust the magnitude and orientations within this top-$r$ subspace~\citep{balazy2024lora,huggingface2023svdtraining}.
However, the drawback of this approach is that retaining only the top singular components can result in the loss of important information, particularly when the singular values distribution is less skewed.
The work most similar to ours is a concurrent effort by \citet{lingam2024svft}, where they introduce various sparsification methods that utilize the SVD of the weights.
However, it is not for self-adaptive LLMs and does not use RL to enhance learning efficiency.

==> tables/compact_ada_tasks.tex <==
\begin{wraptable}{r}{0.5\textwidth}
\centering
\small
\caption{\textbf{Average performance on unseen tasks.} Performance averaged across math, coding, reasoning tasks. Normalized scores are shown in the parentheses.}
\vspace{-3.5mm}
\label{tab:res:compact_svf_ada_tasks}

\begin{tabular}{lccc}
\toprule
\textbf{Method} & \textbf{Llama3-8B} & \textbf{Mistral0.3-7B} & \textbf{Llama3-70B} \\
& \textbf{instruct} & \textbf{instruct} & \textbf{instruct} \\
\midrule
% \multicolumn{4}{l}{\textit{Seen Tasks}} \\
% Base & {\normalsize 66.68 {\footnotesize (\textcolor{gray}{1.00})}} & {\normalsize 47.27 {\footnotesize (\textcolor{gray}{1.00})}} & {\normalsize 85.07 {\footnotesize (\textcolor{gray}{1.00})}} \\
% \quad + LoRA & {\normalsize 68.30 {\footnotesize (\textcolor{green}{1.02})}} & {\normalsize 43.68 {\footnotesize (\textcolor{red}{0.92})}} & {\normalsize 78.16 {\footnotesize (\textcolor{red}{0.92})}} \\
% \quad + \implname & \textbf{{\normalsize 71.92 {\footnotesize (\textcolor{green}{1.08})}}} & \textbf{{\normalsize 62.13 {\footnotesize (\textcolor{green}{1.31})}}} & \textbf{{\normalsize 85.87 {\footnotesize (\textcolor{green}{1.01})}}} \\
% \midrule
\multicolumn{4}{l}{\textit{Unseen Tasks}} \\
Base & {\normalsize 55.38 {\footnotesize (\textcolor{gray}{1.00})}} & {\normalsize 42.69 {\footnotesize (\textcolor{gray}{1.00})}} & {\normalsize 68.98 {\footnotesize (\textcolor{gray}{1.00})}} \\
\quad + LoRA & {\normalsize 51.73 {\footnotesize (\textcolor{red}{0.93})}} & {\normalsize 39.55 {\footnotesize (\textcolor{red}{0.93})}} & {\normalsize 60.96 {\footnotesize (\textcolor{red}{0.88})}} \\
\quad + \implname & \textbf{{\normalsize 57.02 {\footnotesize (\textcolor{green}{1.03})}}} & \textbf{{\normalsize 45.42 {\footnotesize (\textcolor{green}{1.06})}}} & \textbf{{\normalsize 70.11 {\footnotesize (\textcolor{green}{1.02})}}} \\
\bottomrule
\end{tabular}


\end{wraptable}

==> tables/svf_train.tex <==
\begin{table}[!b]
\centering

\caption{Fine-tuning performance of \textsc{LLAMA-3-8B-Instruct} on 4 tasks}

% Results from applying the \svdacro

\small
\begin{tabular}{lllll}
\toprule
 & GSM8K test & MBPP-Pro sub test set & ARC-Easy test & TextVQA sub test set \\
Method &  &  &  &  \\
\midrule
\llama & {\normalsize 75.89 {\footnotesize (\grey{1.00})}} & {\normalsize 64.65 {\footnotesize (\grey{1.00})}} & {\normalsize 88.59 {\footnotesize (\grey{1.00})}} & {\normalsize 37.59 {\footnotesize (\grey{1.00})}} \\
\quad + LoRA & {\normalsize 70.58 {\footnotesize (\red{0.93})}} & \textbf{{\normalsize 67.68 {\footnotesize (\green{1.05})}}} & {\normalsize 88.97 {\footnotesize (\grey{1.00})}} & {\normalsize 45.95 {\footnotesize (\green{1.22})}} \\
\quad + SVF (Ours) & \textbf{{\normalsize 79.15 {\footnotesize (\green{1.04})}}} & {\normalsize 66.67 {\footnotesize (\green{1.03})}} & \textbf{{\normalsize 89.56 {\footnotesize (\green{1.01})}}} & \textbf{{\normalsize 52.31 {\footnotesize (\green{1.39})}}} \\

\midrule
\mistral & {\normalsize 42.83 {\footnotesize (\grey{1.00})}} & {\normalsize 49.50 {\footnotesize (\grey{1.00})}} & {\normalsize 49.50 {\footnotesize (\grey{1.00})}} \\
\quad + LoRA & {\normalsize 36.09 {\footnotesize (\red{0.84})}} & {\normalsize 47.47 {\footnotesize (\red{0.96})}} & {\normalsize 47.47 {\footnotesize (\red{0.96})}} \\
\quad + SVF (Ours) & \textbf{{\normalsize 49.74 {\footnotesize (\green{1.16})}}} & \textbf{{\normalsize 51.52 {\footnotesize (\green{1.04})}}} & \textbf{{\normalsize 85.14 {\footnotesize (\green{1.72})}}} \\

\midrule
\llamaXL & {\normalsize 85.29 {\footnotesize (\grey{1.00})}} & \textbf{{\normalsize 80.81 {\footnotesize (\grey{1.00})}}} & \textbf{{\normalsize 89.10 {\footnotesize (\grey{1.00})}}} \\
\quad + SVF (Ours) & \textbf{{\normalsize 88.32 {\footnotesize (\green{1.04})}}} & \textbf{{\normalsize 80.81 {\footnotesize (\grey{1.00})}}} & {\normalsize 88.47 {\footnotesize (\red{0.99})}} \\

\bottomrule

\end{tabular}
\label{tab:res:svf_train}

\end{table}



==> tables_ws/ablation_few_shots.tex <==

\begin{wraptable}{r}{0.5\textwidth}
\vspace{-4mm}
\caption{\textbf{Few-shot adaptation scaling.} Performance varies with number of examples.
}
% \vspace{-3.5mm}
\centering
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{lc}
\toprule
\textbf{Method} & \textbf{ARC-Challenge} \\
\midrule
\llama & {\normalsize 80.63 {\footnotesize (\grey{1.00})}} \\
\midrule

\quad + 3-shot adaptation & {\normalsize 82.18 {\footnotesize (\green{1.02})}} \\
\quad + 5-shot adaptation & {\normalsize 82.38 {\footnotesize (\green{1.02})}} \\
\quad + 10-shot adaptation & \textbf{{\normalsize 82.61 {\footnotesize (\green{1.02})}}} \\
\quad + 20-shot adaptation & \textbf{{\normalsize 82.61 {\footnotesize (\green{1.02})}}} \\

\bottomrule
\end{tabular}}
\label{tab:ablation:few_shot_adaptation}
\vspace{-10mm}
\end{wraptable}


==> tables_ws/analysis_cross_model_app.tex <==
\begin{table}[!h]
\caption{
\textbf{Cross-model $\boldsymbol{z}$ Vector Transfer.}
Results from transfering the SVF expert vectors trained on \llama to \mistral in the respective training tasks.}
% \vspace{-3.5mm}
\centering
\begin{tabular}{lccc}
\toprule
\textbf{Method} & \textbf{GSM8K} & \textbf{MBPP-pro} & \textbf{ARC-Easy} \\
%\textit{SVF training task} & \small{\textit{GSM8K}} & \small{\textit{MBPP-pro}} & \small{\textit{ARC-Easy}} \\
\midrule

\textsc{Mistral-7B-Instruct-v0.3} & \textbf{{\normalsize 42.83 {\footnotesize (\grey{1.00})}}} & \textbf{{\normalsize 49.50 {\footnotesize (\grey{1.00})}}} & {\normalsize 81.65 {\footnotesize (\grey{1.00})}} \\

\midrule

\quad + Llama SVF (ordered $\sigma_i$) & {\normalsize 42.61 {\footnotesize (\red{0.99})}} & {\normalsize 48.48 {\footnotesize (\red{0.98})}} & \textbf{{\normalsize 81.78 {\footnotesize (\grey{1.00})}}} \\
\quad + Llama SVF (shuffled $\sigma_i$) & {\normalsize 41.93 {\footnotesize (\red{0.98})}} & {\normalsize 46.34 {\footnotesize (\red{0.94})}} & {\normalsize 80.81 {\footnotesize (\red{0.99})}} \\


\bottomrule
\end{tabular}
\label{tab:analysis:cross_model_app}
\end{table}

==> tables_ws/analysis_cross_model_main.tex <==
\begin{table}[!h]
% \vspace{-4mm}
% \caption{\textbf{Cross-model $z$ vector transfer.}
\caption{\textbf{Cross-model $\boldsymbol{z}$ vector transfer.}
Results from transferring the expert vectors trained on \llama to \mistral with cross model few-shot adaptation.
}
% \vspace{-3.5mm}
\centering
\begin{tabular}{lccc}
\toprule
\textbf{Method} & \textbf{MATH} & \textbf{Humaneval} & \textbf{ARC-Challenge} \\
\textit{SVF training task} & \small{\textit{GSM8K}} & \small{\textit{MBPP-pro}} & \small{\textit{ARC-Easy}} \\
\midrule


\textsc{Mistral-7B-Instruct-v0.3} & \textbf{{\normalsize 13.02 {\footnotesize (\grey{1.00})}}} & {\normalsize 43.29 {\footnotesize (\grey{1.00})}} & {\normalsize 71.76 {\footnotesize (\grey{1.00})}} \\

\midrule

\quad + Llama SVF (ordered $\sigma_i$) & {\normalsize 11.96 {\footnotesize (\red{0.92})}} & {\normalsize 45.12 {\footnotesize (\green{1.04})}} & {\normalsize 72.01 {\footnotesize (\grey{1.00})}} \\
\quad + Llama SVF (shuffled $\sigma_i$) & {\normalsize 10.52 {\footnotesize (\red{0.81})}} & {\normalsize 40.24 {\footnotesize (\red{0.93})}} & {\normalsize 70.82 {\footnotesize (\red{0.99})}} \\
\quad + Few-shot adaptation (cross-model) & {\normalsize 12.65 {\footnotesize (\red{0.97})}} & \textbf{{\normalsize 46.75 {\footnotesize (\green{1.08})}}} & \textbf{{\normalsize 75.64 {\footnotesize (\green{1.05})}}} \\

\bottomrule
\end{tabular}
\label{tab:analysis:cross_model_main}
\vspace{-2mm}
\end{table}

==> tables_ws/hyper_p_app.tex <==
\begin{table}[!h]
\centering
\caption{\textbf{Hyper-parameters used for \svdacro and LoRA training.} We perform a sweep on certain sensitive hyper-parameters  across methods for fair comparison.}
% \vspace{-3.5mm}
\begin{tabular}{ll}
\toprule
\multicolumn{2}{c}{\textbf{\svdacro Hyperparameters}} \\
\midrule
Initial mean value of $z$ & $0.1$ \\
Initial variance value of $z$ & $1 \times 10^{-3}$ \\
Global batch size & $256$ \\
Learning rate & $2 \times 10^{-3}$ \\
Clip max norm & $1 \times 10^{-3}$ \\
KL coefficient $\lambda$ & $0.0$, $0.1$, $0.2$, $0.3$ \\
\midrule
\multicolumn{2}{c}{\textbf{LoRA Hyperparameters}} \\
\midrule
Rank & $16$ \\
LoRA alpha & $32$ \\
LoRA dropout & $0.05$ \\
Global batch size & $256$ \\
Learning rate & $1 \times 10^{-5}$, $5 \times 10^{-5}$, $1 \times 10^{-4}$ \\
Clip max norm & $1 \times 10^{-3}$, $1.0$ \\
\bottomrule
\end{tabular}
\label{app:tab:hyperparameters}
\end{table}

==> tables_ws/svf_ada_tasks.tex <==
\begin{table}[!t]
\centering
\vspace{-2mm}
\caption{\textbf{Self-adaptation on unseen tasks.} Normalized scores are in the parentheses.}
% \vspace{-2mm}
\small
\begin{tabular}{llll}
\toprule
Method & MATH & Humaneval & ARC-Challenge \\

\midrule
\llama3 & {\normalsize 24.54 {\footnotesize (\grey{1.00})}} & {\normalsize 60.98 {\footnotesize (\grey{1.00})}} & {\normalsize 80.63 {\footnotesize (\grey{1.00})}} \\
\quad + LoRA & {\normalsize 21.68 {\footnotesize (\red{0.88})}} & {\normalsize 52.44 {\footnotesize (\red{0.86})}} & {\normalsize 81.06 {\footnotesize (\green{1.01})}} \\
\quad + \implname (Prompt) & {\normalsize 25.22 {\footnotesize (\green{1.03})}} & {\normalsize 61.59 {\footnotesize (\green{1.01})}} & {\normalsize 81.74 {\footnotesize (\green{1.01})}} \\
\quad + \implname (Cls-expert) & {\normalsize 25.18 {\footnotesize (\green{1.03})}} & {\normalsize 62.80 {\footnotesize (\green{1.03})}} & {\normalsize 81.37 {\footnotesize (\green{1.01})}} \\
\quad + \implname (Few-shot) & \textbf{{\normalsize 25.47 {\footnotesize (\green{1.04})}}} & \textbf{{\normalsize 62.99 {\footnotesize (\green{1.03})}}} & \textbf{{\normalsize 82.61 {\footnotesize (\green{1.02})}}} \\

\midrule
\mistral & {\normalsize 13.02 {\footnotesize (\grey{1.00})}} & {\normalsize 43.29 {\footnotesize (\grey{1.00})}} & {\normalsize 71.76 {\footnotesize (\grey{1.00})}} \\
\quad + LoRA & {\normalsize 11.18 {\footnotesize (\red{0.86})}} & {\normalsize 31.71 {\footnotesize (\red{0.73})}} & \textbf{{\normalsize 75.77 {\footnotesize (\green{1.06})}}} \\
\quad + \implname (Prompt) & {\normalsize 11.86 {\footnotesize (\red{0.91})}} & {\normalsize 43.90 {\footnotesize (\green{1.01})}} & {\normalsize 72.35 {\footnotesize (\green{1.01})}} \\
\quad + \implname (Cls-expert) & {\normalsize 11.60 {\footnotesize (\red{0.89})}} & {\normalsize 43.90 {\footnotesize (\green{1.01})}} & {\normalsize 74.83 {\footnotesize (\green{1.04})}} \\
\quad + \implname (Few-shot) & \textbf{{\normalsize 13.39 {\footnotesize (\green{1.03})}}} & \textbf{{\normalsize 47.40 {\footnotesize (\green{1.09})}}} & {\normalsize 75.47 {\footnotesize (\green{1.05})}} \\

\midrule
\llamaXL & \textbf{{\normalsize 40.64 {\footnotesize (\grey{1.00})}}} & {\normalsize 78.66 {\footnotesize (\grey{1.00})}} & {\normalsize 87.63 {\footnotesize (\grey{1.00})}} \\
\quad + LoRA & {\normalsize 25.40 {\footnotesize (\red{0.62})}} & {\normalsize 73.78 {\footnotesize (\red{0.94})}} & {\normalsize 83.70 {\footnotesize (\red{0.96})}} \\
\quad + \implname (Prompt) & {\normalsize 40.44 {\footnotesize (\grey{1.00})}} & \textbf{{\normalsize 79.88 {\footnotesize (\green{1.02})}}} & \textbf{{\normalsize 88.48 {\footnotesize (\green{1.01})}}} \\
\bottomrule

\end{tabular}

\label{tab:res:svf_ada_tasks}
\vspace{-6mm}
\end{table}



==> tables_ws/svf_train_tasks.tex <==
% \begin{table}[!t]
% \centering

% \caption{\textbf{LLM Fine-tuning Results.} LLM performance on the test splits.}

% \small
% \begin{tabular}{llll}
% \toprule

% \textbf{Method} & \textbf{GSM8K} & \textbf{MBPP-Pro} & \textbf{ARC-Easy} \\

% \midrule
% \llama & {\normalsize 75.89 {\footnotesize (\grey{1.00})}} & {\normalsize 64.65 {\footnotesize (\grey{1.00})}} & {\normalsize 88.59 {\footnotesize (\grey{1.00})}} \\
% \quad + LoRA & {\normalsize 70.58 {\footnotesize (\red{0.93})}} & \textbf{{\normalsize 67.68 {\footnotesize (\green{1.05})}}} & {\normalsize 88.97 {\footnotesize (\grey{1.00})}} \\
% \quad + SVF (Ours) & \textbf{{\normalsize 79.15 {\footnotesize (\green{1.04})}}} & {\normalsize 66.67 {\footnotesize (\green{1.03})}} & \textbf{{\normalsize 89.56 {\footnotesize (\green{1.01})}}} \\

% \midrule
% \mistral & {\normalsize 42.83 {\footnotesize (\grey{1.00})}} & {\normalsize 49.50 {\footnotesize (\grey{1.00})}} & {\normalsize 49.50 {\footnotesize (\grey{1.00})}} \\
% \quad + LoRA & {\normalsize 36.09 {\footnotesize (\red{0.84})}} & {\normalsize 47.47 {\footnotesize (\red{0.96})}} & {\normalsize 47.47 {\footnotesize (\red{0.96})}} \\
% \quad + SVF (Ours) & \textbf{{\normalsize 49.74 {\footnotesize (\green{1.16})}}} & \textbf{{\normalsize 51.52 {\footnotesize (\green{1.04})}}} & \textbf{{\normalsize 85.14 {\footnotesize (\green{1.72})}}} \\

% \midrule
% \llamaXL & {\normalsize 85.29 {\footnotesize (\grey{1.00})}} & \textbf{{\normalsize 80.81 {\footnotesize (\grey{1.00})}}} & \textbf{{\normalsize 89.10 {\footnotesize (\grey{1.00})}}} \\
% \quad + SVF (Ours) & \textbf{{\normalsize 88.32 {\footnotesize (\green{1.04})}}} & \textbf{{\normalsize 80.81 {\footnotesize (\grey{1.00})}}} & {\normalsize 88.47 {\footnotesize (\red{0.99})}} \\

% \bottomrule
% \end{tabular}

% \label{tab:res:svf_train_tasks}
% \end{table}

% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=\textwidth]{images/vlm_barplot.pdf}
%     % \vspace{-8mm}
%     \caption{\textbf{VLM Results.}
%     }
%     % \vspace{-4mm}
%     \label{fig:vlm_results}
% \end{figure}



\begin{figure}[!b]
    \vspace{-4mm}
    \centering

    % Left side: Table
    \begin{minipage}{0.75\linewidth}
        \centering
        \captionof{table}{\textbf{Fine-tuning results.} LLM performance on the test splits of math, coding and reasoning. Normalized scores are in the parentheses.}
        \vspace{-2mm}
        \small
        \begin{tabular}{llll}
            \toprule
            \textbf{Method} & \textbf{GSM8K} & \textbf{MBPP-Pro} & \textbf{ARC-Easy} \\
            \midrule
            \llama & {\normalsize 75.89 {\scriptsize (\grey{1.00})}} & {\normalsize 64.65 {\scriptsize (\grey{1.00})}} & {\normalsize 88.59 {\scriptsize (\grey{1.00})}} \\
            \quad + LoRA & {\normalsize 70.58 {\scriptsize (\red{0.93})}} & \textbf{{\normalsize 67.68 {\scriptsize (\green{1.05})}}} & {\normalsize 88.97 {\scriptsize (\grey{1.00})}} \\
            \quad + SVF (Ours) & \textbf{{\normalsize 79.15 {\scriptsize (\green{1.04})}}} & {\normalsize 66.67 {\scriptsize (\green{1.03})}} & \textbf{{\normalsize 89.56 {\scriptsize (\green{1.01})}}} \\
            \midrule
            \mistral & {\normalsize 42.83 {\scriptsize (\grey{1.00})}} & {\normalsize 49.50 {\scriptsize (\grey{1.00})}} & {\normalsize 49.50 {\scriptsize (\grey{1.00})}} \\
            \quad + LoRA & {\normalsize 36.09 {\scriptsize (\red{0.84})}} & {\normalsize 47.47 {\scriptsize (\red{0.96})}} & {\normalsize 47.47 {\scriptsize (\red{0.96})}} \\
            \quad + SVF (Ours) & \textbf{{\normalsize 49.74 {\scriptsize (\green{1.16})}}} & \textbf{{\normalsize 51.52 {\scriptsize (\green{1.04})}}} & \textbf{{\normalsize 85.14 {\scriptsize (\green{1.72})}}} \\
            \midrule            
            \llamaXL & {\normalsize 85.29 {\footnotesize (\grey{1.00})}} & \textbf{{\normalsize 80.81 {\footnotesize (\grey{1.00})}}} & \textbf{{\normalsize 89.10 {\footnotesize (\grey{1.00})}}} \\
            \quad + LoRA & {\normalsize 77.26 {\footnotesize (\red{0.91})}} & {\normalsize 68.69 {\footnotesize (\red{0.85})}} & {\normalsize 88.55 {\footnotesize (\red{0.99})}} \\
            \quad + SVF (Ours) & \textbf{{\normalsize 88.32 {\footnotesize (\green{1.04})}}} & \textbf{{\normalsize 80.81 {\footnotesize (\grey{1.00})}}} & {\normalsize 88.47 {\footnotesize (\red{0.99})}} \\
            \bottomrule                
        \end{tabular}
        \label{tab:res:svf_train_tasks}
    \end{minipage}
    \hfill
    % Right side: Figure
    \begin{minipage}{0.23\linewidth}
        \centering
        % \vspace{2mm}
        \includegraphics[width=\linewidth]{images/vlm_barplot.pdf}
        \vspace{-8mm}
        \captionof{figure}{\textbf{Results for the VLM domain.}}
        \label{fig:vlm_results}
    \end{minipage}

\end{figure}


==> tables_ws/table_ablation.tex <==
\begin{table}[h]
% \begin{table}[!b]

% \vspace{-2mm}
\centering
\caption{\textbf{Ablation studies.} We fine-tune \llama on the GSM8K training split with different settings and the results on the test split along with zero-shot transfer results on MATH.
% We highlight the change in learning configurations for better visualization.
%Notably, we set the KL coefficient to 0.1 across all runs utilizing policy gradient for fair comparison.
}
% \vspace{-3.5mm}
% \small
% \begin{tabular}{llllccc}
% \toprule

% \textbf{\#} & \textbf{Method} & \textbf{Objective Function} & \textbf{Module} & \textbf{\#Params ($\downarrow$)} & \textbf{GSM8K ($\uparrow$)} & \textbf{MATH ($\uparrow$)} \\

% \midrule
% 0 & \multicolumn{4}{c}{\textsc{LLAMA-3-8B-Instruct}} & {75.89 {\scriptsize (\grey{1.00})}} & {24.54 {\scriptsize (\grey{1.00})}} \\ 
% \midrule

% 1 & \svdacro & Policy gradient & MLP & 0.39M & { 78.62 {\scriptsize (\green{1.04})}} & {24.20 {\scriptsize (\green{0.99})}} \\

% 2 & \svdacro & Policy gradient & \cellcolor{gray!20}{attention} & \textbf{0.16M} & {76.19 {\scriptsize (\green{1.00})}} & {24.20 {\scriptsize (\green{0.99})}} \\

% 3 & \svdacro & Policy gradient & \cellcolor{gray!20}{MLP + attention} & 0.58M & \textbf{{ 79.23 {\scriptsize (\green{1.04})}}} & \textbf{{25.04 {\scriptsize (\green{1.04)}}}} \\

% 4 & \svdacro & \cellcolor{gray!20}{Next token pred} & attention & \textbf{0.16M} & { 60.50 {\scriptsize (\green{0.80})}} & {18.52 {\scriptsize (\green{0.75})}} \\

% 5 & \cellcolor{gray!20}{LoRA} & Policy gradient & attention & 6.82M & { 57.92 {\scriptsize (\green{0.76})}} & {15.72 {\scriptsize (\green{0.64})}} \\

% \bottomrule
% \label{tab:res:ablation}
% \end{tabular}

% \vspace{-8mm}
% \end{table}

% \vspace{-3.5mm}
\small
\begin{tabular}{llllccc}
\toprule

\textbf{\#} & \textbf{Method} & \textbf{Objective Function} & \textbf{Module} & \textbf{\#Params ($\downarrow$)} & \textbf{GSM8K ($\uparrow$)} & \textbf{MATH ($\uparrow$)} \\

\midrule
0 & \multicolumn{4}{c}{\textsc{LLAMA-3-8B-Instruct}} & {75.89 {\scriptsize (\grey{1.00})}} & {24.54 {\scriptsize (\grey{1.00})}} \\ 
\midrule

1 & \svdacro & Policy gradient & MLP & 0.39M & { 78.62 {\scriptsize (\green{1.04})}} & {24.20 {\scriptsize (\green{0.99})}} \\

2 & \svdacro & Policy gradient & attention & \textbf{0.16M} & {76.19 {\scriptsize (\green{1.00})}} & {24.20 {\scriptsize (\green{0.99})}} \\

3 & \svdacro & Policy gradient & MLP + attention & 0.58M & \textbf{{ 79.23 {\scriptsize (\green{1.04})}}} & \textbf{{25.04 {\scriptsize (\green{1.04)}}}} \\

4 & \svdacro & Next token pred & attention & \textbf{0.16M} & { 60.50 {\scriptsize (\green{0.80})}} & {18.52 {\scriptsize (\green{0.75})}} \\

5 & LoRA & Policy gradient & attention & 6.82M & { 57.92 {\scriptsize (\green{0.76})}} & {15.72 {\scriptsize (\green{0.64})}} \\

\bottomrule
\label{tab:res:ablation}
\end{tabular}

\vspace{-5mm}
\end{table}


